Logical Reasoning for Higher-Order Functions with Local State

We introduce an extension of Hoare logic for call-by-value higher-order functions with ML-like local reference generation. Local references may be generated dynamically and exported outside their scope, may store higher-order functions and may be used to construct complex mutable data structures. This primitive is captured logically using a predicate asserting reachability of a reference name from a possibly higher-order datum and quantifiers over hidden references. We explore the logic's descriptive and reasoning power with non-trivial programming examples combining higher-order procedures and dynamically generated local state. Axioms for reachability and local invariant play a central role for reasoning about the examples.

==> reply_second.tex <==
Dear Referees, 

We thank you very much again for your time spent reading our
submission and your further very useful suggestions. We 
corrected our paper following your valuable advice.

Below we answer each point independently raised by the referee reports.

Nobuko Yoshida
Kohei Honda
Martin Berger

----------------------------------------------------------------------------
%% Referee no 1:
----------------------------------------------------------------------------

%%  * This is an excellent paper and can be accepted for Logical Methods in Computer Science as it is

%% Did the authors submit their answers to the reviews, in addition to
%% the actual revisions? That would be helpful in seeing what's going on.

We had submitted the answer to your first referee report. 
Unfortunately, during the resubmission process, it was accidentally 
not sent to you. 

We attach the first reply to you. This reply includes 
the third and fourth points of your questions. 

Additional materials:

Regarding to the third point:

-- page 9, before Notation 2.1, 
   the paragraph starting ``Note that expression...''
-- page 10, Section 2.3 Second Item !e_1 = !e_2 is included  

Regarding to the forth point: 

-- Theorem 5.10 (page 32) gives the full proof in Appendix C.5 
-- We list your example for the elimination after Theorem 5.10. 

Our first reply in the following contains more detailed explanation. 

---------------------------------------------------------------------
> I have found the paper to be an interesting, albeit at moments a very
> challenging reading. The presented logic, just like the logics from
> the author's previous papers, contains a plethora of propositional
> connectives and inference rules with quite involved semantics. After
> some time, one is left wondering if it is possible to somehow
> consolidate this logic into one which will be much easier to describe,
> understand and use.

> However, it must be said that a lot of this complexity may stem just
> from the inherent difficulty of the subject matter itself, and the
> authors deserve credit for carrying out the development.

> With this in mind, I recommend the acceptance of the paper. I do,
> however, have a few concerns, which I would like the authors to
> address before the publication.

---

Thank you for your important questions. We appreciate them and have 
added those points discussed below in the updated submission.

> My first question concerns the definition 3.1. on page 11.  This
> definition introduces the notion of a model, and the first thing it
> assumes is that the context Gamma does not contain free variables of
> type ref. 

In the initial submission, there was a confusion in the use of Delta
(which was a mapping from locations to types in Gamma) in Def 3.1. We
have simplified the definition. Gamma contains free
variables of reference types. The semantics is intended to give
meaning to assertions on open program (which naturally contain free
variables of reference types).

For example, 

(nu l)(x:l\cdot y:l', [l -> 3]\cdot [l' -> 3])

is a model with a typing environment: 

Gamma = {x:Ref(\nat),y:Ref(\nat),l':Ref(Nat)}

> When I first saw this definition, I thought this restriction
> looked a bit harsh, and I couldn't quite justify it to myself. Reading
> on, however, showed that the authors themselves do not respect this
> restriction. The first example comes at the end of page 11 in equation
> (3.6) where x and y are variables of type ref. Also, Section 3.7 on
> page 17 starts with a similar "cheat", where the semantics of content
> quantification assumes that \epsilon(x)=l, which would seem to assume
> that x is of ref type. Similarly, Section 5.3 on page 28 uses a model
> with free ref variables x and x' to show a counterexample of the
> implication C->nu x.C.
> 
> Are these really correct uses of the definition, or am I missing
> something? If the later is true, then I would certainly appreciate a
> more prominent comment in the paper, just to avoid any confusion.
>

By changing our definition, these examples now conform to the definition
of the models.

---

> My second question concerns the inference rule [Ref] from Figure 1 on
> page 22. This rule captures the semantics of the operator ref for
> generating a fresh reference. The freshness of the reference is
> established by requiring that it cannot reach any existing datum i of
> type X. However, the rule does not use any explicit quantification
> over i, but rather, the uses of the rule are allowed to explicitly
> instantiate this variable i as they see fit. I found this a bit
> troublesome, for the following reasons. 
> 
> First of all, it is clear that we can apply this rule twice (or more)
> to produce conclusions with two different i's. But how can we then
> collect these two (or more) different conclusions in order to show
> that the newly generated ref is different from the two (or more)
> existing data? 
> 
> Is it sufficient to just put these two different data
> into a pair (or a tuple), and substitute the pair for i? Is it
> possible to build this tuple if some of its parts are hidden?

By choosing a fresh (hence distinct) variable each time,
we can treat such consecutive reference generation. We
illustrate by an example whose assertions do not use the power 
of freshness fully but would suffice for illustration. First
we can infer:

(1)   {truth} Ref(0):_m {!m=0 and m\neq i} @ \emptyset

(2)   {!m=0 and m\neq i} Ref(0):_n {!n=!m=0 and n\neq j} @ \emptyset

(where we take off \nu by axioms: we also relaxed the
predicate for unreachability to inequality). From (2) we 
obtain:

(2')  {!m=0 and m\neq i} Ref(0):_n {!m=!n=0 and n\neq m}

where j in (2) is replaced by m (this is how we can
"collect" distinct freshness) by the proof rule (Subs)
in Figure 6 (page 46 in the submission version, now placed
in Figure 6): 

       {C}M:_u {C'} u\not\fpn(e)
(subs) ----------------------------------------
       {C{e/i}}  M:_u {C'{e/i}}

Let the postcondition of (2') be G. Now we use:

       {C}M:_m {C_0}   {C_0}N:_n {C'[(m, n)/u]}
(pair) ----------------------------------------
                 {C} (M, N):_u {C'}
 
to obtain the pair has the postcondition 

        G {pi_l(u) / m} {pi_r(u) / n}

Since (subs) rule is significant but was not emphasised as much as
should be in the initial submission, we have placed it among the main
rules and have added the illustration of this point. 

> One would think that a rule similar to Hoare's rule of conjunction
> would be necessary to handle this correctly, but I couldn't find such
> a rule in the paper or in the appendices. 
> 
> How practical is this rule? In order to use it, we basically need to
> collect all the existing program data, hidden or not. This may not only
> be very cumbersome if a lot of data is present in the program, but may
> also be non-compositional. That is, assume that we already proved a
> correctness of some program using the rule [Ref]. What happens when we
> put that program into a larger context, which introduces new data? 

We already discussed how this can be done through our discussions
above, using fresh variables for each sequent which treats a new
reference generation. In fact, we (can) usually replace fresh
variables with appropriate expressions through [Subs] immediately
after the new name generation (in the example above, we can
consider the simpler version of (2) whose precondition is say
Truth, can apply [Subs], then use [Inv] to obtain (2')), in which
case we even do not worry about name clash. This is also the case
when (as is often the case in practice) the new reference
generation is treated via Let-Ref rule. This rule allows us to
directly treat partial disjointness (for example part of a datum
to be disjoint from part of another datum etc.) compositionally, 
as discussed through examples in Section 6.

See also the next discussion on the treatment of these variables
in a large proof tree.

> One would think that the existing proof must be changed in order to
> account for freshness with respect to this new data. Hence, strictly
> speaking, the current logic does not let us build libraries of
> *verified* programs, because old proofs must be retrofitted for new
> contexts. I should mention here that working around this particular
> point is precisely why separation logic was invented.

In the context of the preceding discussions, the authors
understand the referee's point as follows: suppose we
infer, for each sub-program that generates a fresh
reference, a relatively strong assertion which uses these
"fresh" variables.  If so, since the names of fresh
variables can overlap, we need to rename them in order to
avoid their name clash so as to use, for example, [subs] 
appropriately.

We do not consider this is a limitation of the present method,
fundamentally and practically, for the following reasons.

(a) Fundamentally, the [Ref] and [LetRef] rules allow partial
sharing of newly generated references (which is hard to do, for
example through separation), which is explicit in the induced
letref rule. For example, in order to specify the behaviour
(effect) of a program such as

    let y=Ref(2) in ( z:=y ; lambda x.(x+!y) )

which results in a hidden, fresh location, which is nevertheless
reachable from $y$ and the returned closure, or in order to
specify the behaviour of programs which generate or manipulate
general graphs, we need to logically treat partial sharing,
which is enabled by these constructs.

(b) Practically fresh names introduced thus, can be treated
as special names which are virtually bound at the sequent
level (semantically they are in fact bound at the sequent
level, just as auxiliary variables in Hoare logic via
Kleymann's rule). Such a binding can also be realised in
e.g. editors, proof assistant, etc., as for the standard
auxiliary variables.  In addition, in practice we can often
dispense with this freshness by instantiating fresh
variables to appropriate expressions immediately after
creation of references, as we already discussed before.

It may also be noted that there is a clean translation of 
this treatment of new reference generation into an 
underlying process logic..

* * *

As to the comparison with separation conjunction, there are two
basic points which need be observed. Firstly, we note that the
orientations are quite different, so we need be careful about
comparisons. For example, SL does not allow

          {truth} x:=x {truth} 

where x is in the heap. This point is also discussed in our
previous paper [JFP07].

Secondly, to our knowledge, various versions of SL do not
have a notion of hidden reference (which is fundamental for
correspondence with observational semantics) nor,
relatedly, the general treatment of partial reachability,
which is essential to specify programs which treat (say)
general graphs. In contrast, the presented logic enables a
uniform treatment of not only data structures based on
strict separation but also those which are based on graphs
and stored functions with shared local data.  Some such
points are now illustrated in Section 6 of the updated
submission, when we compare SL and other logics to the
present approach.

> The above comments are also applicable in the example from section
> 6.1, page 32. Here the authors use the rule [Ref] to move from step 3
> to step 4 in the derivation. Some comment here on the fact that the
> derivation is actually context-dependent would be
> appreciated. Otherwise, we could just take \tile{e} to be the empty
> tuple, right?

As to the use of the derived sequent in a larger proof (context),
we have already discussed above: the variable i can be replaced by 
any fresh variable. 

The use of general \tilde{e} is *essential* in this case since the
[LetRef] rule embodies the idea that we can start from total
disjointness (separation) and reach possibly partial disjointness
in the conclusion. For this purpose we need to have explicit
x#\tilde{e} initially, which may possibly be weakened in the
post-condition C through the actions in N.

These points are added in Section 5 with LetRef rule. 

> Same comments also apply to located judgements from Section 4.3. That
> is, what happens if the effect set wants to mention hidden data. Is
> that allowed, and why is it compositional in the above sense?

We thank the referee for pointing this out since this is a significant
point which should have been illustrated better. The power of located
assertions (especially vis-vis the corresponding rule in original
Hoare logic or those which use say separating conjunction) is that,
regardless of the effects being at hidden references or not, we can
soundly apply the invariant rule: hidden or free, if a reachable store
is altered, we put it in a write set (note also a new reference generation 
per se does not have any semantic effect, e.g. let x=Ref(2) in () is 
the same as () observationally).

As an illustration of this point, suppose an effect is in a hidden
location which is stored in r (hence reachable from r), then by 
using the de-reference notation, we can write:

             f y = z {C'} @ !r

where !r is interpreted in the pre-state (in the submission, 
we prohibit the use of de-reference in a write set to avoid 
confusion as to where it should be interpreted: however this 
does not lose generality since we can write the assertion above 
as: \exists i.(!r=i and f y = z {C'} @ i).

The use of hidden references in a write set can be extended
to the case when a write set is represented by a formula
denoting an indefinite set of references.

We added a few lines clarifying this point in the paper (Section 4.4). 

---

> My third question concerns Theorem 5.9 on elimination. The theorem
> states that if all reachability predicates in C are finite (that is,
> do not contain an arrow type or a type variable), then C can be
> rewritten into C' which does not contain any reachability
> predicates. 

> Would you please demonstrate this theorem on the example of the
> predicate
> 
>    x --> y 
> 
> where x:ref ref int and y:ref int. There are no arrow types here or
> type variables, but I don't see how to remove the reachability
> predicate x --> y. What am I missing? 
> 

If we have x-->y and if they are finite then we may assume, for 
example:

         x of type ref(ref(ref(alpha)))
         y of type ref(alpha)

As in this example, the key point of having types is that a
reachability relation is dictated by types: this is why the
elimination works.  In the example above, the reachability
from x to y can simply be decomposed into: 

         !!x=y.

We have also added the full proof of this theorem in the 
new submission, in Appendix C.4.

---

> Fourth question: What exactly goes wrong in the definition of
> expressions e of the assertion logic (page 7), if you allowed that
> lambdas are expressions? Is there no use in your logic for comparing
> functions for equality? Can we actually avoid this? 

We first answer the questions raised above directly. If we
enlarge the terms in the present logical language to encompass
arbitrary programs, then terms in the logic will have effects
when we evaluate them (such as lambda y.x:=3). We also do not
wish to add the equation such as () = (x:=3), noting the
right-hand side is of the unit type. And, if we do not allow
such side effect as part of terms, it is hard to construct
interesting lambda expressions. We also note that if we include
applications lambda expressions, it leads to non-termination.
We wish to make terms to be effect-less and terminated ones,
allowing the use of equality, quantification, etc. as in the
standard first-order logic. Thus if two variables representing
functions are equated then they can be mutually replaceable. How
this is *practically* useful can be seen in our assertion and
reasoning for IncShared in Section 6.

Secondly, the tenet of the present logic is to represent observable
behaviour of programs, not their internal structures.  We want
assertions for programs to be independent from programs' text. In
this way we obtain substitutability: if we have a derivation for a
conclusion {C}M:_u{C'} and in that derivation we use, for a
subprogram N of M, {A}N:_x{B}, and if we also have {A}N':_x{B},
then we can replace N with N' in M, still satisfying the same
precondition C and the same postcondition C'. Note this
substitutability is also a basis of such engineering usage of the
program logic as design-by-contract.

>If we had e1,e2:ref(a->b), can we write the proposition !e1 = !e2?

If e1, e2 are terms defined in our syntax in Section 2.2, we can
write !e1 = !e2. Note neither e_1 nor e_2 contains lambda
expressions: and this equality obeys the standard axioms for 
equations and quantification.


---

> Some typos:

Many thanks for pointing these out: we have corrected all of them.

> - page 3, "at the end the program incShared" --> "at the end of the
>   program incShared".

> - page 7, "together satisfying C'" --> "together satisfying C"

> - page 14, "M1[u:v] =/= M1[u:w]" should be "M2[u:v] =/= M2[u:w]"

> - page 16, "Note that even the type" --> "Note that even if the type"

> - page 30, equation (5.10) lacks a parenthesis at the end




%% A new typo:

%% On page 12, the authors revised their statement of Definition 3.1. to
%% address the question that I asked of. They simply removed the first
%% sentence, but now the second sentence alone should read "An open
%% model..." instead of "Then an open model...".

corrected.

--------------------------------------------------------------------------
%% Referee no 2:
--------------------------------------------------------------------------
%%  * The paper can be accepted for Logical Methods in Computer Science after minor revisions.

%% The points raised in the review have been addressed satisfactorily in
%% the revised version; the paper can now be accepted.  The authors may
%% wish to take into account some further comments on minor details made
%% below. Generally, I found the authors' reply to the review extremely
%% helpful; the authors may wish to incorporate parts of this material
%% into the paper more literally than they already have. (E.g. I can see
%% that part of the very illuminating discussion of hiding
%% vs. disjointness has become Example 10 in Sec. 2.3 on p.10, but at
%% this time, the reader has already been wondering about hidden
%% locations in models since page 6.)

Thank you very much. We included more from our first reply 
such as the pointer to Sec 2.3 from page 6, explanaiton of 
the consequence rule and the relative completeness. 

%% Some more details:

%% p.4 bottom: scope extrusion

Done

%% Last line before Sec. 2: reasoning *about*

Done

%% Remark 3.4: matters --&#62; matter, evaluates --&#62; evaluate; confusion
%% involving 2 and 3.

Done

%% Ref. 49: "1997, reprinted from LICS'06" sounds impossible.

Corrected

%% Related work, evaluation logic: this remains slightly unclear. E.g. is
%% it really the case that evaluation logic is about equality of
%% programs? This seems to be the focus of Moggi's original work on the
%% computational lambda-calculus, but evaluation logic talks about
%% properties of states reached after execution of a program, not about
%% equality. Secondly, evaluation logic includes variables representing
%% programs, so that one is not actually forced to write full programs in
%% formulas (incidentally, it should be pointed out at the time of
%% introducing the logical language that terms are not programs, and
%% why); moreover, genericity over the underlying programming language is
%% precisely one of the key points of evaluation logic. At any rate, this
%% does not look like one of the main differences between your work and
%% evaluation logic, which I would tend to pinpoint more along lines like
%% operational vs. denotational and specific vs. generic, with your
%% contribution being to cover specific language features like local
%% state.

Modified as suggested.  

%% References: Conference proceedings should be properly cited with
%% conference namReferences: Conference proceedings should be properly cited with
%% conference name (not just the abbreviation), series, publisher, and
%% year (e.g. Logic in Computer Science, LICS 2006, IEEE, 2006,
%% pp. XXX-XXX; or Fundamental Approaches to Software Engineering, FASE
%% 2008, LNCS, vol XXXX, Springer, 2008, pp. XXX-XXX). Journal names
%% should be abbreviated according to standard (e.g. AMS or ACM)
%% conventions, and not by acronyms -- e.g. "Theoret. Comput. Sci.", not
%% "TCS".

Corrected. For some reason, the publishers of the journals do not appear 
in LMCS format. We shall find out later. 

%% Some new occurrences of omitted "about" after "reasoning" (e.g. p.44)

Done. 

Many thanks for your detailed review. 



